On Divergence Measures for Bayesian Pseudocoresets

A Bayesian pseudocoreset is a small synthetic dataset for which the posterior over parameters approximates that of the original dataset. While promising, the scalability of Bayesian pseudocoresets is not yet validated in realistic problems such as image classification with deep neural networks. On the other hand, dataset distillation methods similarly construct a small dataset such that the optimization using the synthetic dataset converges to a solution with performance competitive with optimization using full data. Although dataset distillation has been empirically verified in large-scale settings, the framework is restricted to point estimates, and their adaptation to Bayesian inference has not been explored. This paper casts two representative dataset distillation algorithms as approximations to methods for constructing pseudocoresets by minimizing specific divergence measures: reverse KL divergence and Wasserstein distance. Furthermore, we provide a unifying view of such divergence measures in Bayesian pseudocoreset construction. Finally, we propose a novel Bayesian pseudocoreset algorithm based on minimizing forward KL divergence. Our empirical results demonstrate that the pseudocoresets constructed from these methods reflect the true posterior even in high-dimensional Bayesian inference problems.

==> tables/cifar10-ipc1-main.tex <==
\begin{table}
\centering

\caption{HMC and SGHMC performances of Bayesian pseudocoresets with the size of 1 image per class on CIFAR10 test dataset. Aug means whether to use image augmentations in pseudocoresets training. All values are averages over ten random seeds on training HMC and SGHMC.\\}
\label{tab:cifar10-ipc1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc} 
\hline
\multirow{2}{*}{} & \multicolumn{2}{c}{HMC (no aug)}                                       & \multicolumn{2}{c}{HMC (with aug)}                                         & \multicolumn{2}{c}{SGHMC (with aug)}                                      \\ 
\cline{2-7}
                  & acc ($\uparrow$)              & nll ($\downarrow$)            & acc ($\uparrow$) & nll ($\downarrow$) & acc ($\uparrow$)              & nll ($\downarrow$)             \\ 
\hline
Random            & $0.1745\spm{0.0084}$          & $2.4507\spm{0.0657}$          & $0.1745\spm{0.0084}$           &  $2.4507\spm{0.0657}$                               & $0.1414\spm{0.0045}$          & $2.9798\spm{0.0725}$           \\
BPC-rKL           & $0.2472\spm{0.0120}$          & $2.1635\spm{0.0327}$          & $0.2416\spm{0.0133}$          &  $2.1688\spm{0.0486}$                               & $0.2162\spm{0.0083}$          & $2.4617\spm{0.0841}$           \\
BPC-W             & $\mathbf{0.3435}\spm{0.0207}$ & $\mathbf{1.9311}\spm{0.0329}$ & $0.3338\spm{0.0158}$          &  $1.9589\spm{0.0265}$                               & $\mathbf{0.2934}\spm{0.0121}$ & $\mathbf{2.1400}\spm{0.0333}$  \\
BPC-fKL           & $0.3354\spm{0.0066}$          & $2.0253\spm{0.0311}$          & $\mathbf{0.3468}\spm{0.0119}$           & $\mathbf{1.9574}\spm{0.0269}$                                & $0.2823\spm{0.0128}$          & $2.1426\spm{0.0343}$           \\
\hline
\end{tabular}%
}
\end{table}

==> tables/cifar10-ipc10-main.tex <==
% \usepackage{multirow}
\begin{table}
\centering
\caption{HMC and SGHMC performances of Bayesian pseudocoresets with the size of 10 images per class on CIFAR10 test dataset. Aug means whether to use image augmentations in pseudocoresets training. All values are averages over ten random seeds on training HMC and SGHMC.\\}
\label{tab:cifar10-ipc10}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc} 
\hline
\multirow{2}{*}{} & \multicolumn{2}{c}{HMC (no aug)}                                       & \multicolumn{2}{c}{HMC (with aug)} & \multicolumn{2}{c}{SGHMC (with aug)}                                      \\ 
\cline{2-7}
                  & acc ($\uparrow$)              & nll ($\downarrow$)            &acc ($\uparrow$)  &nll ($\downarrow$)                      & acc ($\uparrow$)              & nll ($\downarrow$)             \\ 
\hline
Random            & $0.2807\spm{0.0050}$          & $2.1070\spm{0.0178}$          &$0.2807\spm{0.0050}$  &$2.1070\spm{0.0178}$                      & $0.3085\spm{0.0077}$          & $2.1953\spm{0.0481}$           \\
BPC-rKL           & $0.3253\spm{0.0075}$          & $1.9627\spm{0.0312}$          &$0.3017\spm{0.0074}$  & $2.0251\spm{0.0134}$                     & $0.3789\spm{0.0154}$          & $1.9492\spm{0.0605}$           \\
BPC-W             & $0.3535\spm{0.0127}$          & $1.9450\spm{0.0258}$          &$0.3646\spm{0.0082}$  & $1.9307\spm{0.0171}$                     & $\mathbf{0.4890}\spm{0.0172}$ & $1.6971\spm{0.0392}$           \\
BPC-fKL           & $\mathbf{0.4294}\spm{0.0101}$ & $\mathbf{1.7292}\spm{0.0248}$ &$\mathbf{0.4252}\spm{0.0091}$  & $\mathbf{1.7334}\spm{0.0217}$                     & $0.4878\spm{0.0103}$          & $\mathbf{1.6762}\spm{0.0390}$  \\
\hline
\end{tabular}%
}
\end{table}

==> tables/cifar10-ipc20-main.tex <==

\begin{table}
\centering
\caption{HMC and SGHMC performances of Bayesian pseudocoresets with the size of 20 images per class on CIFAR10 test dataset. Aug means whether to use image augmentations in pseudocoresets training. All values are averages over ten random seeds on training HMC and SGHMC.\\}
\label{tab:cifar10-ipc20}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc} 
\hline
\multirow{2}{*}{} & \multicolumn{2}{c}{HMC (no aug)}            & \multicolumn{2}{c}{HMC (with aug)}          & \multicolumn{2}{c}{SGHMC (with aug)}         \\ 
\cline{2-7}
                  & acc ($\uparrow$)     & nll ($\downarrow$)   & acc ($\uparrow$)     & nll ($\downarrow$)   & acc ($\uparrow$)     & nll ($\downarrow$)    \\ 
\hline
Random            & $0.3292\spm{0.0057}$ & $2.0164\spm{0.0212}$ & $0.3292\spm{0.0057}$ & $2.0164\spm{0.0212}$ & $0.3832\spm{0.0070}$ & $1.8999\spm{0.0338}$  \\
BPC-rKL           & $0.3686\spm{0.0115}$ & $1.8848\spm{0.0338}$ & $0.3518\spm{0.0102}$ & $1.9540\spm{0.0350}$ & $0.4307\spm{0.0073}$ & $1.8555\spm{0.0263}$  \\
BPC-W             & $0.4546\spm{0.0146}$ & $1.7336\spm{0.0325}$ & $0.4606\spm{0.0200}$ & $1.7334\spm{0.0506}$ & $\mathbf{0.5691}\spm{0.0167}$ & $\mathbf{1.5439}\spm{0.0408}$  \\
BPC-fKL           & $\mathbf{0.4910}\spm{0.0088}$ & $\mathbf{1.6279}\spm{0.0264}$ & $\mathbf{0.4833}\spm{0.0069}$ & $\mathbf{1.6440}\spm{0.0231}$ & $0.5153\spm{0.0093}$ & $1.6701\spm{0.0256}$  \\
\hline
\end{tabular}%
}
\end{table}

==> tables/pm-advance.tex <==
\begin{table}[t]
\caption{BPC-fKL ipc10 gaussian noise vs sghmc, sghmc is better}
\centering
\begin{tabular}{lcc}
\hline
          & \multicolumn{2}{c}{SGHMC} \\ \cline{2-3} 
          & acc         & nll         \\ \hline
sgd+noise & $0.4878\spm{0.0103}$            &  $1.6762\spm{0.0390}$           \\
sghmc     & $\mathbf{0.5020}\spm{0.0165}$            &  $\mathbf{1.6561}\spm{0.0585}$           \\ \hline
\end{tabular}

\label{tab:pm-advance}
\end{table}

==> tables/table.tex <==

\begin{table}[t]
\caption{ipc10}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
                       &    & \multicolumn{2}{c}{no aug ( both train and test)} & \multicolumn{2}{c}{aug (both train and test)} & \multicolumn{2}{c}{Aug in train, no aug in test(previous)} \\ \cmidrule(l){3-8} 
                       &    & acc                     & nll                     & acc                   & nll                   & acc                            & nll                           \\ \midrule
\multirow{2}{*}{SGD}   & tm & 0.5204                  & \textbf{1.4007}         & \textbf{0.6155}       & \textbf{1.1749}       & \textbf{0.5237}                & \textbf{1.4017}               \\
                       & pm & \textbf{0.5376}         & 1.4255                  & 0.5914                & 1.2887                & 0.5194                         & 1.4856                        \\ \midrule
\multirow{2}{*}{HMC}   & tm & 0.3872                  & 2.0918                  & -                     & -                     & 0.4138                         & 2.0422                        \\
                       & pm & \textbf{0.4320}         & \textbf{1.9668}         & -                     & -                     & \textbf{0.4383}                & \textbf{1.9547}               \\ \midrule
\multirow{2}{*}{SGHMC} & tm & -                       & -                       & 0.4894                & 1.7006                & -                              & -                             \\
                       & pm & -                       & -                       & \textbf{0.4900}       & \textbf{1.6756}       & -                              & -                             \\ \bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[t]
\caption{ipc1}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
                       &    & \multicolumn{2}{c}{no aug ( both train and test)} & \multicolumn{2}{c}{aug (both train and test)} & \multicolumn{2}{c}{Aug in train, no aug in test(previous)} \\ \midrule
                       &    & acc                     & nll                     & acc                   & nll                   & acc                            & nll                           \\ \midrule
\multirow{2}{*}{SGD}   & tm & \textbf{0.4005}         & \textbf{1.7855}         & \textbf{0.4343}       & \textbf{1.878}        & 0.3704                         & \textbf{1.8736}               \\
                       & pm & 0.3838         & 1.9006                  & 0.3999                & 2.324                 & \textbf{0.377}                 & 1.9471                        \\ \midrule
\multirow{2}{*}{HMC}   & tm & \textbf{0.3493}         & \textbf{1.9249}         & -                     & -                     & \textbf{0.3447}                & \textbf{1.9359}               \\
                       & pm & 0.3171         & 2.0783         & -                     & -                     & 0.3419                         & 1.9854                        \\ \midrule
\multirow{2}{*}{SGHMC} & tm & -                       & -                       & \textbf{0.3092}       & \textbf{2.1553}       & -                              & -                             \\
                       & pm & -                       & -                       & 0.3031       & 2.1582       & -                              & -                             \\ \bottomrule
\end{tabular}%
}
\end{table}
